Enabling Long-term Fairness in Dynamic Resource Allocation

We study the fairness of dynamic resource allocation problem under the $\alpha$-fairness criterion. We recognize two different fairness objectives that naturally arise in this problem: the well-understood slot-fairness objective that aims to ensure fairness at every timeslot, and the less explored horizon-fairness objective that aims to ensure fairness across utilities accumulated over a time horizon. We argue that horizon-fairness comes at a lower price in terms of social welfare. We study horizon-fairness with the regret as a performance metric and show that vanishing regret cannot be achieved in presence of an unrestricted adversary. We propose restrictions on the adversary's capabilities corresponding to realistic scenarios and an online policy that indeed guarantees vanishing regret under these restrictions. We demonstrate the applicability of the proposed fairness framework to a representative resource management problem considering a virtualized caching system where different caches cooperate to serve content requests.

==> old.tex <==
% \section{Nash Bargaining}
% The Nash Bargaining Solution (NBS), proposed in the seminal paper~\cite{Nash1950}, is an axiomatic fairness criterion for dispersing to a set of  players/actors/entities the benefits (or gains) of their cooperation. Simply put, this theory tries to answer the question: how should we split the cooperation gains so as to entice the players to agree to join their endeavors and improve their aggregate outcome/performance/utility? The basic premise here is that whenever the players cooperate, they achieve performance that exceeds the sum of the individual performances they achieve when operating independently. This latter is also known as the disagreement point (vector, in particular). 

% In the context of computing systems, for instance, imagine that two cloud computing companies with different types of servers, process the computing loads of their clients independently, each of them achieving a certain performance in terms of processing time or induced costs. If, however, they interconnect their servers, then due to the complementary of their equipment and the diversity of their users requests, they can reduce their total costs and improve the processing delays. This creates a surplus (compared to the case they serve their clients independently), and the question is how to split it. One natural way is of course to split the benefits in a egalitarian fashion, i.e., equally among the 2 companies. Another way is to split them in a utilitarian way~\cite{Andreu1995}, i.e., to give more to the company ``in need'' (whatever that means). Going a step further, one can extend this question to: how to operate the joined servers? E.g., how to configure them, how many hours to run each of them, etc. Should we operate them so as to maximize the total performance (utilitarian approach)? Or, should we minimize the costs of, e.g., the most ``weak'' company? Again, this can be answered by solving a properly formulated Nash Bargaining Problem that, in this expanded version, will not only determine how to split the gains but actually will shape these gains in the first place (e.g., switching off many servers from one company impacts the total delay for both). 

% Clearly, these ideas are not unique to NBS since many other fairness criteria/frameworks try to address them. However, NBS comes from the area of cooperative game theory, and it is self enforcing, i.e., the players will actually agree to apply this solution without the need for an external authority to enforce compliance (unlike centrally-enforced fairness criteria). How do we know that the players will agree? Well, it is an axiomatic theory (hence, Nash just assumed it), but also has been verified with various behavioral experiments. Now, interestingly, Nash proved that this point can be found by solving a specific quasi-convex program that takes as input the disagreement points. NBS has been extensively applied in communication networks, e.g., see~\cite{Boche2011} for transmission power control,~\cite{Iosifidis2017} for mobile Internet sharing among wireless users,~\cite{Wenjie2009} for content delivery in ISP-CDN partnerships, and~\cite{Liang2017} for cooperative caching in information-centric networks. NBS has numerous applications in all kinds of problems. 

% However, to the best of our knowledge, it is only considered as a static problem: we know the utility functions, the cooperation gains, and the decision space, and we try to solve the optimization problem, taking into account the specifics of each domain/problem. But, what happens when all these are unknown or time-varying? When the utility functions and the potential cooperation gains change from slot to slot, or when we need to make splitting decisions without even knowing the gains? To put it simply, we need to answer the question: 

% \emph{How can we distribute the benefits of cooperation when these are a priori unknown and potentially time-varying in an unpredictable way? Can we provide guarantees to the players that they will indeed enjoy an NBS-compliant performance despite these dynamics?}
% \subsection{Nash Bargaining Solution's Desiderata}
% \label{s:nbs_desiderata}
% The Nash bargaining solution has the following desirable (axiomatic) properties~\cite{Nash1950,Andreu1995}:
% \begin{itemize}
%     \item \textbf{Pareto Optimality:} NBS is Paretian, i.e., there is no other feasible solution which yields a
% better payoff than the NBS for one user, and no worse payoff for all other users.
%     \item \textbf{Individual Rationality:} Offers to each user a payoff that is no worse than the payoff it has
% when does not participate in the bargaining game (disagreement point).
%     \item \textbf{Independence from Utility Units and Origins:} If we apply an affine transformation to the players’ utility functions or change the absolute scale of utilities, then the initial solution can yield the corresponding bargaining solution for the new problem under the same transformation. This property ensures that the resource allocation is independent of the way we measure the players’ utilities.

%     \item \textbf{Independence of Irrelevant Alternatives:} If the set of solutions shrinks without affecting the eligibility of the bargaining outcome, then the latter remains unchanged.
%     \item \textbf{Symmetry:} Whenever the set of feasible cooperation solutions is symmetric, i.e., it remains unaltered under permutation of axes, then all components of NBS are equal. This implies that if all players are identical, then the cooperation gains are split equally.
% \end{itemize}


% % \section{Related Work}

